Quantum Phase Transitions and Dynamics in Perturbed Flatbands

In recent years, there has been a growing interest in flatband systems which exhibit macroscopic degeneracies. These systems offer a valuable mathematical framework for the extreme sensitivity to perturbations and interactions. This sensitivity unveils a wide variety of exotic and unconventional physical phenomena. Moreover, the progress in their experimental realization contributes to the expanding landscape of exploration in this field. This thesis aims to summarize all the works throughout the Ph.D. program. Firstly, an in-depth exploration was conducted on the impact of weak quasiperiodic perturbations on one-dimensional two-band all-bands-flat lattices. These tight-binding Hamiltonian are diagonalized through a sequence of local unitary transformations. By adjusting the quasiperiodic potential parameters, the key achievement involves finding a critical-to-insulator transition and identifying fractality edges in the flatband systems with quasiperiodic perturbations. Next, the investigation delved into the effects of on-site interactions among hard-core bosons in one- and two-dimensional cross-stitch lattices. One key finding is that groundstate energy primarily depends on compact localized states. Moreover, the presence of barriers of compact localized states trap bosons, leading to the emergence of non-ergodic excitation and Hilbert space fragmentation. Lastly, a compact localized eigenstate of the one-dimensional diamond chain using an electric circuit was successfully generated via local (linear and non-linear) driving. This achievement opens up a versatile circuit platform for the generation of flatbands and holds promise for potential applications in the field of quantum information. I hope these collective efforts have expanded the frontiers of the field and made a meaningful contribution to the scientific community.

==> committee.tex <==
\begin{center}
    \textbf{\huge We hereby approve the Ph.D of Ihor Vakulchyk}
\end{center}

\vskip 50pt

\begin{center}
    \textbf{December 2021}
\end{center}

\vskip 80pt


\begin{center}
    \underline{\kern 250pt sign }
    
    Chairman of Thesis Committee
    
        \underline{\kern 250pt sign }
    
    Thesis Committee Member
    
            \underline{\kern 250pt sign }
    
    Thesis Committee Member
    
            \underline{\kern 250pt sign }
    
    Thesis Committee Member
    
            \underline{\kern 250pt sign }
    
    Thesis Committee Member
    
            \underline{\kern 250pt sign }
    
    Thesis Committee Member
    
            \underline{\kern 250pt sign }
    
    Thesis Committee Member
\end{center}

\vskip 50pt

\begin{center}
    \textbf{\large{UNIVERSITY OF SCIENCE AND TECHNOLOGY}}
\end{center}

==> remarks.tex <==
% =========================================================================== %
% =========================================================================== %
% REMARK COLLECTIONS
% =========================================================================== %
% =========================================================================== %
\noindent\textcolor{blue}{Remarks from Alexei : First draft}

\begin{itemize}[leftmargin=*]\itemsep0em
\item General remarks ::
\begin{itemize}[leftmargin=*]\itemsep0em
\item improve the text -- perhaps with Joel's help (if possible)?
\item use simpler phrasing?
\item reread carefully and make sure internal references are correct, e.g. link the chapters, not refer to your publications
\item introduction to the chapters better be more specialised to the topic of the chapter
\item do not refer to your published papers, but rather to the respective chapters
\end{itemize}
\item More specific remarks ::
\begin{itemize}[leftmargin=*]\itemsep0em
\item Better thesis title? \shlee{SL : Edited}
\item Improve the abstract
\item Eq. 1.1: unclear \shlee{SL : Answered}
\item Sec. 1.1: constructive vs destructive interference is very confusing! \shlee{SL : Edited}
\item After Eq. 1.6: there is definitely more to add on various previous studies of FB
\item Is Fig. 1.3 references in the text (and other figures)? 
\item I think Sec. 1.3 and 1.4 can be merged together \shlee{SL : Edited}
\item There are forward references to wavepacked spreading -- perhaps could be avoided? \shlee{SL : Edited}
\end{itemize}
\end{itemize}
